EvoGroup: A Self-Evolving Harness for Group Agents in Shared Contexts

With the rise of Group Agent such as Claude Tag, agents increasingly serve as digital workers for long-term team collaboration. These agents operate over shared contexts that continuously accumulate through multi-user interactions. However, existing agent memory systems are mainly designed for individual users and struggle to capture group-level knowledge in shared contexts, including group relationships and collaboratively formed knowledge. Manual memory strategies further limit adaptation to diverse and evolving shared contexts. To this end, we propose \textbf{EvoGroup (EvoG)}, a self-evolving harness for group agents that starts from a minimal six-tool cold start and adapts through interaction with shared context. EvoG uses confidence and task outcomes to select informative trajectories, while also eliciting self-reflections on uncertainty in low-confidence cases. The analysis agent then examines selected trajectories through adaptive progressive disclosure, followed by bucketed analysis to synthesize high-level findings that guide the evolve agent in revising the Harness. Empirically, pass@1 on held-out split of EverMemBench improves from 71.07\% to 89.58\%, surpassing both self-evolving memory and human-designed harnesses, including Claude Code (85.83\%). To evaluate generalization, we freeze the evolved harness and evaluate it on the unseen GroupMemBench, where, with GPT-5.5, it demonstrates effective generalization and outperforms both memory baselines and human-designed harnesses.

==> case_study.tex <==
\RequirePackage{tcolorbox}
\tcbuselibrary{breakable,skins,raster}

% ---- palette (four-box cards, kept for compatibility) ----------------------
\definecolor{egCaseBlue}{RGB}{70,130,180}
\definecolor{egCaseGreen}{RGB}{34,139,34}
\definecolor{egCaseBrown}{RGB}{139,69,19}
\definecolor{egCaseViolet}{RGB}{138,43,226}

% ---- palette (trajectory cards, sage scheme) -------------------------------
\definecolor{egTrajBar}{RGB}{120,149,144}      % card title bar
\definecolor{egTrajFrame}{RGB}{141,162,157}    % outer frame
\definecolor{egTrajEdge}{RGB}{201,212,209}     % thin inner rule
\definecolor{egTrajInk}{RGB}{38,48,51}         % block labels
\definecolor{egTrajUser}{RGB}{239,243,242}
\definecolor{egTrajThink}{RGB}{240,242,241}
\definecolor{egTrajCall}{RGB}{236,244,247}
\definecolor{egTrajResp}{RGB}{238,243,239}
\definecolor{egTrajSum}{RGB}{241,246,242}
\definecolor{egTrajHarness}{RGB}{246,249,248}

% ---- shared card geometry ---------------------------------------------------
\tcbset{caseinner/.style={%
  enhanced,
  width=\linewidth,
  boxsep=1pt,
  left=4pt,
  right=4pt,
  top=2pt,
  bottom=2pt,
  arc=1.5pt,
  boxrule=0.55pt,
  before skip=0pt,
  after skip=0pt,
  fontupper=\small,
}}

\newtcolorbox{caseframe}[1]{%
  enhanced,
  breakable,
  pad at break*=0pt,
  title after break={#1\quad\normalfont\small(continued)},
  width=\textwidth,
  colback=white,
  colframe=egTrajEdge,
  boxrule=0.8pt,
  arc=2pt,
  boxsep=1pt,
  left=6pt,
  right=6pt,
  top=3pt,
  bottom=6pt,
  before skip=8pt,
  after skip=0pt,
  title={#1},
  fonttitle=\small\bfseries,
  coltitle=white,
  colbacktitle=egTrajBar,
  toptitle=2.5pt,
  bottomtitle=2pt,
  lefttitle=5pt,
  righttitle=5pt,
  halign title=left,
}

% ============================================================================
% Trajectory cards
% ============================================================================
\tcbset{trajinner/.style={%
  enhanced,
  width=\linewidth,
  boxsep=1pt,
  left=4pt,
  right=4pt,
  top=1.5pt,
  bottom=1.5pt,
  arc=2pt,
  boxrule=0.55pt,
  before skip=1.5pt,
  after skip=0pt,
  halign=left,
  fontupper=\footnotesize\linespread{1.02}\raggedright,
}}

\newtcolorbox{caseuser}{%
  trajinner,
  colback=egTrajUser,
  colframe=egTrajEdge,
  before upper={\textbf{Question:}\enspace},
}

\newtcolorbox{casethink}{%
  trajinner,
  colback=egTrajThink,
  colframe=egTrajEdge,
  before upper={\textcolor{egTrajInk}{\ttfamily\bfseries <think>}\par\vspace{1pt}},
}

\newtcolorbox{casetool}{%
  trajinner,
  colback=egTrajCall,
  colframe=egTrajEdge,
  fontupper=\ttfamily\scriptsize\linespread{1.0}\raggedright,
  before upper={\textcolor{egTrajInk}{\ttfamily\bfseries <tool\_call>}\par\vspace{1pt}},
}

\newtcolorbox{caseresp}{%
  trajinner,
  colback=egTrajResp,
  colframe=egTrajEdge,
  fontupper=\ttfamily\scriptsize\linespread{1.0}\raggedright,
  before upper={\textcolor{egTrajInk}{\ttfamily\bfseries <tool\_response>}\par\vspace{1pt}},
}

\newtcolorbox{caseanswer}{%
  trajinner,
  colback=egTrajSum,
  colframe=egTrajEdge,
  before upper={\hyphenpenalty=10000\exhyphenpenalty=10000\textcolor{egTrajInk}{\bfseries Assistant Summary:}\par\vspace{1pt}},
}

\newtcolorbox{caseharness}{%
  trajinner,
  colback=egTrajHarness,
  colframe=egTrajEdge,
  before upper={\textbf{Harness $\Delta$}\enspace},
}

% ============================================================================
% Legacy four-box cards (no longer used by appendix_cases.tex)
% ============================================================================
\newtcolorbox{casetrace}{%
  caseinner,
  colback=egCaseGreen!8,
  colframe=egCaseGreen!55,
  before upper={\textbf{Trace}\par\vspace{1pt}}
}

\newtcolorbox{caseedit}{%
  caseinner,
  colback=egCaseBrown!8,
  colframe=egCaseBrown!55,
  before upper={\textbf{Harness Edit}\par\vspace{1pt}}
}

\newtcolorbox{casequery}{%
  caseinner,
  colback=egCaseBlue!8,
  colframe=egCaseBlue!55,
  before upper={\textbf{Query and Revised Trace}\par\vspace{1pt}}
}

\newtcolorbox{casemechanism}{%
  caseinner,
  colback=egCaseViolet!8,
  colframe=egCaseViolet!55,
  before upper={\textbf{Mechanism}\par\vspace{1pt}}
}

